The Impact of Cosmic Rays on Thermal and Hydrostatic Stability in Galactic Halos

We investigate how cosmic rays (CRs) affect thermal and hydrostatic stability of circumgalactic (CGM) gas, in simulations with both CR streaming and diffusion. Local thermal instability can be suppressed by CR-driven entropy mode propagation, in accordance with previous analytic work. However, there is only a narrow parameter regime where this operates, before CRs overheat the background gas. As mass dropout from thermal instability causes the background density and hence plasma $\beta \equiv P_g/P_B$ to fall, the CGM becomes globally unstable. At the cool disk to hot halo interface, a sharp drop in density boosts Alfven speeds and CR gradients, driving a transition from diffusive to streaming transport. CR forces and heating strengthen, while countervailing gravitational forces and radiative cooling weaken, resulting in a loss of both hydrostatic and thermal equilibrium. In lower $\beta$ halos, CR heating drives a hot, single-phase diffuse wind with velocities $v \propto (t_\mathrm{heat}/t_\mathrm{ff})^{-1}$, which exceeds the escape velocity when $t_\mathrm{heat}/t_\mathrm{ff} \lesssim 0.4$. In higher $\beta$ halos, CR forces drive multi-phase winds with cool, dense fountain flows and significant turbulence. These flows are CR dominated due to "trapping" of CRs by weak transverse B-fields, and have the highest mass loading factors. Thus, local thermal instability can result in winds or fountain flows where either the heat or momentum input of CRs dominates.

==> junk.tex <==
\section{Analytic Considerations} \label{sec:theoretical_considerations}


\subsection{Thermal Instability in Stratified Medium with CR (Short version)} \label{subsec:TI_cr_heat}





%Observations of cool core clusters and the inner CGM show that their cooling times are much shorter than the lifespan of these objects, so a `cooling flow' where gas cools catastrophically and infalls should occur. No such flows were observed, thus there must be a heating source maintaining thermal equilibrium. AGN feedback and thermal conduction \citep{guo08_global_stab} have been proposed as possible sources, and simulations have shown they can indeed suppress cooling flows. Such a global thermal balance, however, does not rule out possibilities of a local thermal instability, and it was shown through observations of $H\alpha$ filaments and low-ions that cold clouds do exist in galaxy clusters and halos.




\subsection{Thermal Instability in Stratified Medium with CR (Long version)} \label{subsec:TI_cr_heat_long}

\chad{Shoot, I'm not sure which version I like more...the long version has nice details but seems too long. Maybe you can move some of the discussion, for instance some of the comparison to Butsky et al., to a later Discussion section? In either the short or long version, I'd suggest making it even more clear that CR heating causes two things: 1) modifications to linear stability, 2) propagating modes. Maybe one way to do this is to create a separate subsection called "Effects of CR Heating"? } \navin{I am leaning towards the short section as it seems more readable. I should probably move some of the discussion in the long version to the discussion and the mathematical details to the appendix. I added a summary section at the end of the short version the two effects from CR heating.}
In this section we review briefly thermal instability in a stratified medium, highlighting the contributions from CR heating. We consider the coupled limit of the CR-MHD equations, i.e. the CR flux has the steady-state form (eqn.\ref{eqn:cr_flux_steady_state}) and terms involving $\bm{\sigma}_c\cdot\qty[\vb{F}_c - \qty(E_c + P_c)\vb{v}]$ become $-\nabla P_c$. In this limit CRs transfer momentum and energy to the gas at the rates given by eqn.\ref{eqn:coupled_momentum_transfer} and \ref{eqn:coupled_energy_transfer} respectively.

Thermal gas cools radiatively and the cooling term $\mathcal{C}$ can be written as
\begin{equation}
    \mathcal{C} = \rho^2\Lambda\qty(T), \label{eqn:coolin_term}
\end{equation}
where $T = P_g/\rho$ is the gas temperature, related to $P_g$ and $\rho$ via the ideal gas law (we have absorbed the Boltzmann constant and the mean molecular mass). For parameters relevant to galaxy halos and clusters, the cooling function $\Lambda\qty(T)$ can be approximated as power laws with index $\Lambda_T \equiv\pdv*{\ln{\Lambda}}{\ln{T}} = -2/3$ and $1/2$ respectively. 

Observations of cool core clusters and the inner CGM show that their cooling times are much shorter than the lifespan of these objects, so a `cooling flow' where gas cools catastrophically and infalls should occur. No such flows were observed, thus there must be a heating source maintaining thermal equilibrium. AGN feedback and thermal conduction \citep{guo08_global_stab} have been proposed as possible sources, and simulations have shown they can indeed suppress cooling flows. Such a global thermal balance, however, does not rule out possibilities of a local thermal instability, and it was shown through observations of $H\alpha$ filaments and low-ions that cold clouds do exist in galaxy clusters and halos.

In unstratified local thermal instability, hot gas that has been cooled slightly becomes denser, causing it to cool faster. This cooling runaways and in-situ cold clouds are formed. Cold clouds formed this way are usually small in scale ($l\ll c_s t_\mathrm{cool}$) and isobaric, i.e. $\delta P_g\approx 0$, but experience sharp increase in densities. The conditions for isobaric thermal instability to occur is that the cooling index $\Lambda_T$ be less than an order unity positive number, and the cold clouds be of size greater than the Field's length, which demarcates the regime where conduction restores thermal balance faster than the cooling time.

Large patches of dense gas of scale $l\gg c_s t_\mathrm{cool}$ in pressure equilibrium with the surroundings can also be thermally unstable if the cooling rate increases with lower temperature, i.e. $\Lambda_T < 0$ (e.g. in galaxy halos, where $\Lambda_t\approx -2/3$). Cold clouds formed this way are usually isochoric, i.e. $\delta\rho\approx 0$, because there is not enough time for the cooling gas to maintain pressure equilibrium, which occurs over a sound crossing time. 

In a stratified medium, there is an additional condition $t_\mathrm{cool}/t_\mathrm{ff}\lesssim 10$ required for non-linear cold clouds to be formed \citep{mccourt_ti_stratified,singh15_sperical_ti}. $t_\mathrm{cool}$ is the cooling time, defined by
\begin{equation}
    t_\mathrm{cool} = \frac{P_g}{\qty(\gamma_g - 1)\rho^2\Lambda}, \label{eqn:cooling_time}
\end{equation}
while $t_\mathrm{ff}$ is the free-fall time, defined by
\begin{equation}
    t_\mathrm{ff} = \sqrt{\frac{2 h}{g}}, \label{eqn:ff_time}
\end{equation}
where $h$ is the height. The reason for this condition is due to non-linear mode coupling with buoyant oscillations. It is fundamentally a non-linear result, which does not appear in linear stability calculations. Density fluctuations were found to saturate at 
\begin{equation}
    \frac{\delta\rho}{\rho} = 0.1\qty(\frac{t_\mathrm{cool}}{t_\mathrm{ff}})^{-1}. \label{eqn:hydro_saturate}
\end{equation}

With magnetic fields, the density fluctuations saturate instead at \citep{ji18_ti}
\begin{equation}
    \frac{\delta\rho}{\rho} = 3\beta^{-1/2}\qty(\frac{t_\mathrm{cool}}{t_\mathrm{ff}})^{-1}, \label{eqn:mhd_saturate}
\end{equation}
where $\beta=8\pi P_g/B^2$ is the plasma $\beta$. The MHD density fluctuations approach the hydrodynamic case when $\beta\rightarrow 900$, but below that MHD density fluctuations are enhanced, the reason being that magnetic fields can suppress buoyant oscillations, lessening non-linear mode coupling. This effect is independent of the orientation of the field lines.

Recently, \citet{butsky20_ti_cr} simulated the effect of CRs on stratified thermal instability and found that it can provide non-thermal support for clouds against collapse, increasing their sizes and the overall cold mass fraction. This also allows small clouds to form isochorically instead of isobarically, as in the previous cases, thus the density fluctuations in the presence of CRs saturate at a lower level. However, they have considered only a background where the magnetic field is perpendicular to $\nabla P_c$, thus CR heating comes only from perturbations (see eqn.\ref{eqn:coupled_energy_transfer}, there is no CR heating if $\vb{v}_s\perp\nabla P_c$) and its impact on linear stability is still yet to be simulated. \chad{A main goal of this paper is study CR-modified thermal instability when stratification and the magnetic field are aligned.}

If the magnetic field is aligned with the direction of stratification, there could be significant background CR heating. The effects of CR heating on linear thermal instability has been detailed in \citet{kempski20_thermal_instability}, we briefly review them in the following, considering exclusively the case where the magnetic field aligns with gravity. In particular, beginning from the purely hydro case, we describe the effects of CRs on local thermal instability in the limits $l\ll c_s t_\mathrm{cool}$ and $l\gg c_s t_\mathrm{cool}$. The mathematical details have been relegated to Appendix.\ref{app:linear}, here we recapitulate the main points.

For $l\ll c_s t_\mathrm{cool}$, pressure balance must be maintained. Previously this meant $\delta P_g\approx 0$ (i.e. isobaric) as only thermal gas can provide pressure support. With CRs we now require $\delta P_\mathrm{tot} = \delta P_g + \delta P_c \approx 0$, which does not preclude the possibility that $\delta P_g = -\delta P_c\neq 0$. A closer look at the linearized CR-MHD equations shows that $\delta P_g\neq 0$ is possible when CR pressure dominates ($\alpha\gg 1$) and diffusion is weak. In this case $\delta P_g/P_g\gg\delta\rho/\rho$ as well, i.e. isochoric, and would explain why \citet{butsky20_ti_cr} saw a decrease in $\delta\rho/\rho$ at CR dominated regimes. Physically the modes can be isochoric because CR pressure, being dominant, can counteract any $\delta P_g$ to maintain $\delta P_\mathrm{tot}\approx 0$. However, if diffusion is strong, $\delta P_c$ will be suppressed and isochoric modes would be impossible. Unbeknowest to \citet{butsky20_ti_cr}, (\chad{I'd re-word "unbeknownst" or take it out}) in the CR dominated regime with background CR heating, CRs do work against Alfven waves and cause the modes the travel at speed $\propto v_A$ up the $P_c$ gradient (see, for example, eqn.29 of \citet{kempski20_thermal_instability}). For small $\alpha$, $\delta P_g = -\delta P_c \approx 0$ is still true, thus the modes are still isobaric.

For $l\gg c_s t_\mathrm{cool}$, there is not enough time for pressure balance to be restored and cooling happens isochorically. Unlike the $l\ll c_s t_\mathrm{cool}$ limit where the role of maintaining pressure balance can be partitioned among the gas and CRs, there is no such counterpart to $\delta\rho$, so large scale modes, if thermally unstable, must cool isochorically. Nevertheless, if CR dominates and diffusion weak, work done on the Alfven waves can still cause the modes to travel at $\propto v_A$ up the CR pressure gradient.

The nature of the unstable modes in different parameter regimes $\alpha,\omega_d/\omega_A,\beta,\Lambda_T$ (where $\omega_d = \kappa_\parallel (\vu{b}\cdot\vb{k})^2$ and $\omega_A = \vb{k}\cdot\vb{v}_A$) is displayed in Fig.1, which shows the characteristics of the thermal modes from solving the linear eigenvalue problem (Appendix ?). We plotted only the small scale limit ($l\ll c_s t_\mathrm{cool}$) as large clouds, if thermally unstable, can only cool isochorically and present less complexity in terms of linear theory. They are also susceptible to shattering as the cloud gas pressure drops, causing surrounding gas to collapse on itself and breaking up into smaller cloudlets \citep{mccourt18_shattering,gronke20_mist_cloud}. In the figures we have demarcated isochoric modes from the isobaric with thick dashed green lines. The $\alpha-\omega_d/\omega_A$ parameter space can in general be divided into three regions: A diffusion dominated background $\xi > 1$, represented by the space under the $\xi\sim 1$ line. The streaming dominated background $\xi < 1$, represented by the space above the $\xi\sim 1$ line, can be divided into a CR dominated case $\alpha > 1$ and otherwise. In agreement with the discussion above, unstable modes falling under the $\xi\sim 1$ line are isobaric as CR diffusion suppresses $\delta P_c$. Isochoric modes are possible in a streaming dominated background provided $\alpha > 1$ while in the $\alpha < 1$ case cooling can only be isobaric.

Stability is in general determined by three dimensionless numbers: The cooling index
\begin{equation}
    \Lambda_T \equiv \pdv{\ln{\Lambda}}{\ln{T}}, \label{eqn:cooling_index}
\end{equation}
the ratio of CR pressure to gas pressure
\begin{equation}
    \alpha = \frac{P_c}{P_g}, \label{eqn:pc_pg}
\end{equation}
and
\begin{equation}
    \xi = \frac{\kappa_\parallel}{\alpha t_\mathrm{cool} v_A^2}, \label{eqn:stream_dominance}
\end{equation}
which in some cases can be interpreted as the ratio of the background CR diffusive to streaming flux\footnote{The background CR streaming flux is given by $F_\mathrm{c,st}\sim P_c v_A$ while the diffusive flux is given by $F_\mathrm{c,diff}\sim\kappa_\parallel\nabla P_c$. The ratio of the diffusive to streaming flux is $\kappa\nabla P_c/P_c v_A$. In a background where cooling is substantially balanced by CR heating, $v_A\nabla P_c\sim \rho^2\Lambda$. Substituting $\nabla P_c$ from this balance into the ratio gives $\kappa_\parallel/\alpha t_\mathrm{cool} v_A^2$, i.e. $\xi$. If CR heating is subdominant compared to radiative cooling this interpretation of $\xi$ as the ratio of diffusive to streaming flux would not be accurate.}. Similar to the pure hydro case, isochoric modes can be unstable only if $\Lambda_T < 0$ while isobaric modes can be unstable as long as $\Lambda_T$ is less than an order unity positive number (typically $\sim 2$). CRs affect the stability of the modes through CR heating, in particular, if the perturbed CR heating is in phase and stronger than the perturbed cooling, thermal instability is suppressed. Concentrating again in the small scale limit ($l\ll c_s t_\mathrm{cool}$), the perturbed CR heating is given by
\begin{equation}
    \delta\qty(-\vb{v}_A\cdot\nabla P_c) = -i\omega_A\delta P_c, \label{eqn:pert_cr_heat} 
\end{equation}
while the perturbed cooling is
\begin{equation}
    \delta\qty(-\rho^2\Lambda) = -\rho^2\Lambda\qty(2 - \Lambda_T)\frac{\delta\rho}{\rho} - \rho^2\Lambda\Lambda_T\frac{\delta P_g}{P_g}. \label{eqn:pert_cool}
\end{equation}
If the background is in thermal equilibrium, local thermal stability is then determined by the perturbed CR heating and cooling. Their ratio in the isobaric ($\delta P_g/P_g\ll\delta\rho/\rho$) and isochoric ($\delta P_g/P_g\gg\delta\rho/\rho$) cases are
\begin{equation}
    \frac{\delta\qty(\textrm{CR Heating})}{\delta\qty(\mathrm{Cooling})} =
    \begin{cases}
        \frac{i\omega_A}{\qty(2 - \Lambda_T)\omega_c}\frac{\delta P_c/P_g}{\delta\rho/\rho} & \textrm{Isobaric} \\
        \frac{i\omega_A}{\omega_c\Lambda_T} & \textrm{Isochoric},
    \end{cases}
    \label{eqn:ratio_cr_heat_cool}
\end{equation}
where $\omega_c = \rho^2\Lambda/P_c$ is the cooling rate and we have used $\delta P_c \approx -\delta P_c$ in the isochoric case. 

In the isochoric case, the perturbed CR heating is always $\pi/2$ out of phase with cooling, thus they don't directly cancel each other. The effect of CR heating in this case is to cause the modes to oscillate and propagate at frequency $\propto\omega_A$ up the CR pressure gradient, as \citet{kempski20_thermal_instability} has shown. Stability is then determined only by whether $\Lambda_T < 0$ or not, as in the hydro case.

In the isobaric case, CR heating can suppress cooling if there is an out of phase component between $\delta P_c$ and $\delta\rho$. CR diffusion can provide this phase shift. In the strong diffusion limit where $\omega_d\gg\omega_A$ (or equivalently $k \kappa_\parallel/v_A\gg 1$), $\delta P_c$ will scale as $\delta P_c/P_g\sim i (\alpha\omega_A/\omega_d) (\delta\rho/\rho)$, i.e. shifted by a phase of $\pi/2$ from $\delta\rho$. Substituting this into eqn.\ref{eqn:ratio_cr_heat_cool} gives
\begin{equation}
    \frac{\delta\qty(\textrm{CR Heating})}{\delta\qty(\mathrm{Cooling})} \sim -\frac{\alpha v_A^2 t_\mathrm{cool}}{\kappa_\parallel} = -\xi^{-1}, \label{eqn:ratio_fast_diff}
\end{equation}
where the minus sign indicates the opposite nature of CR heating and cooling. Clearly, if the background is diffusion dominated ($\xi > 1$), the perturbed CR heating cannot suppress cooling and vice versa. For weak diffusion $\omega_d\ll\omega_A$ the out of phase component between $\delta P_c$ and $\delta\rho$ does not have a simple mathematical form, but physically it should be difficult to suppress cooling if the CR pressure were weak ($\alpha\ll 1$, less CR heating). For $\alpha\gg 1$ unstable modes are isochoric. Suppression is possible for $\alpha\sim 1$ provided the time to diffuse CR across a wavelength is shorter than the cooling time $\omega_d/\omega_c\gtrsim 1$, in another words $\lambda\lesssim\sqrt{\kappa_\parallel t_\mathrm{cool}}$.

In fig.\ref{fig:stability} we colormapped the growth rate of the unstable thermal mode on the left column and the ratio of perturbed CR heating to cooling on the right. In agreement with the discussion above, unstable isobaric modes occur at where CR heating is less than cooling. This happens when $\xi > 1$ or $\alpha\ll 1$. For the $\xi < 1$ and $\alpha\sim 1$ regime suppression occurs for diffusion that is neither too strong nor too weak, as demonstrated by the dip in the stability threshold in the figure. Isochoric modes cannot be suppressed by CR heating, but can so if $\Lambda_T > 0$. For weaker magnetic field, CR heating is also weaker, thus the parameter regime where modes are CR heating suppressed shrinks.

Buoyantly, $\delta\rho/\rho$ may not be an appropriate indication of the presence of cold gas as cold cloud formation is increasingly isochoric the more dominant CR pressure is. Saturation should be less sensitive to $t_\mathrm{cool}/t_\mathrm{ff}$ as isochoric cold clouds can levitate for a longer time. These claims were confirmed by \citet{butsky20_ti_cr} in a series of increasingly CR dominant simulations (up to $\alpha = 10$), which showed decreasing $\delta\rho/\rho$ but a larger cold mass fraction for higher $\alpha$. Despite the lower sensitivity of the cold mass fraction to $t_\mathrm{cool}/t_\mathrm{ff}$, there is still a noticeable drop as $t_\mathrm{cool}/t_\mathrm{ff}$ transitions across 1 because the modes are not perfectly isochoric (at least up to $\alpha = 10$, the highest $\alpha$ they simulated). No cold clouds were observed at $t_\mathrm{cool}/t_\mathrm{ff}$ of 10 or above. They have however considered only the case where the magnetic field is perpendicular to the direction of stratification, thus there were no background CR heating and they did not observe suppression of thermal modes due to CR heating, neither did they observe propagation of the modes up the $P_c$ gradient $\propto v_A$.

What would happen if the modes were to propagate? One can envisage in the halo or cluster medium a CR infused region of size $\sim L$ where $t_\mathrm{cool}$ is small and conditions favorable for thermal instability, elsewhere $t_\mathrm{cool}$ might be too long to produce in-situ cold clouds. For instance, this would be the case for a cored NFW profile \citep{navarro97_nfw_prof}, $t_\mathrm{cool}/t_\mathrm{ff}$ is low only for some radius range around $r_\mathrm{core}$. If the time it takes a mode to cool through thermal instability to non-linear amplitudes (some multiple of $t_\mathrm{cool}$) is longer than the time $t_\mathrm{cross} = L/v_\mathrm{ph}$ it takes to transverse the region (where $v_\mathrm{ph}$ is the phase velocity of the mode), then cold gas formation would be suppressed. That is, the ratio
\begin{equation}
    \theta \equiv \frac{t_\mathrm{cool}}{t_\mathrm{cross}} \label{eqn:chi_def}
\end{equation}
should indicate whether cold gas can be formed. In particular, if $\theta \gtrsim 1$ suppression due to this transverse effect should occur. From linear theory, \citet{kempski20_thermal_instability} has found that the phase velocity of the thermal modes
\begin{equation}
    v_\mathrm{ph} \sim
    \begin{cases}
        \alpha v_A & P_c/P_g \lesssim 1 \\
        v_A & P_c/P_g \gg 1.
    \end{cases}
    \label{eqn:phase_velocity}
\end{equation}
Note that this effect is does not appear in linear stability analysis but is theorized by comparing two timescales.

As a short summary, if CRs were present and there is background CR heating, small scale isochoric modes are possible. CR heating can suppress isobaric thermal instability by counteracting cooling provided that diffusion is neither too strong (such that $\xi > 1$ and $\delta P_c$ is suppressed) nor too weak (such that $\delta P_c$ can diffuse out of phase with $\delta\rho$ before the gas is cooled). The isochoric nature of the modes can lead to higher cold mass fraction and less sensivity to $t_\mathrm{cool}/t_\mathrm{ff}$. In theory the propagation of these modes limits the time for cooling to become non-linear and can suppress the cold mass fraction.

\subsection{CR transport and the bottleneck effect} \label{subsec:bottleneck}

\begin{figure}
    \centering
    \includegraphics[width=0.48\textwidth]{bottle_profile_nobump.png}
    \caption{CR pressure ($P_c$) under various transport models in an exponentially decreasing density background (black dashed line). $\eta$ denotes the ratio of diffusive to streaming flux, so the higher $\eta$ is, the more diffusive the CRs are. Increasing $\eta$ allows more CRs to escape outwards and provide pressure support.}
    \label{fig:nobump}
\end{figure}

\begin{figure}
    \centering
    \includegraphics[width=0.48\textwidth]{one_bottle.png} \\
    \includegraphics[width=0.48\textwidth]{bottle_profile.png}
    \caption{\emph{Top:} Bottleneck effect with one bump. The density is initiated with a single bump at $x=1.5$ in an otherwise smoothly decreasing profile (black dashed curve). The CR pressure $P_c$ is also smoothly decreasing initially (blue curve). CRs streaming from the left bottleneck at the bump due to decrease in Alfven speed, causing CR pressure to build up like water filling up a bucket, i.e. CR pressure rises in a leveled manner. $P_c$ eventually settles in a staircase-like structure (orange curve), with a sharp jump tracing the falling side of the bump and a flat plateau before it. For illustration only the CR variables are evolved, all the gas variables (density, gas pressure, velocity, magnetic field) are held fixed. \emph{Bottom:} Bottleneck effect with multiple bumps at various values of $\eta$, the ratio of the diffusive to streaming flux. $\eta$ is a function of $x$ (decreasing with $x$ in fact), the displayed values of $\eta$ are taken at $x=0$. A multi-step staircase, similar to that demonstrated in \citet{tsung21_staircase}, can be seen. The staircase structure is smoothed as $\eta$ increases beyond 1.}
    \label{fig:one_bottle}
\end{figure}

\chad{The transition from 2.2 to 2.3 seems a little abrupt. Wonder if you should motivate the bottleneck more by first asking "can CR heating hold up an atmosphere? This depends on the overall magnitude and location of heating, which depend on the relative contributions of streaming vs diffusive transport. This is especially interesting in the limit of streaming dominated transport due to the so-called bottleneck effect"...something like that. } \navin{Added.}

Can CR hold up an atmosphere? This depends on the overall magnitude and location of CR pressure support and heating, which depend on the relative contributions of streaming vs diffusive transport. This is especially interesting in the limit of streaming dominated transport due to the so-called bottleneck effect. In the absence of CR diffusion, the CR energy eqn.\ref{eqn:cr_energy} mandates at steady state that along the magnetic field,
\begin{equation}
    P_c\qty(v + v_A)^{\gamma_c} = \mathrm{const}. \label{eqn:bottleneck}
\end{equation}
For a static fluid this reduces to
\begin{equation}
    P_c\rho^{-\gamma_c/2} = \mathrm{const}. \label{eqn:bottleneck_reduce}
\end{equation}
That is, the CR pressure rises/drops with density. Therefore, in streaming dominated flows the CR and density scale-heights are related by $L_c = 3 L_\rho/2$\footnote{The density and CR scale-heights are defined respectively by $L_c = P_c/|\nabla P_c|$ and $L_\rho = \rho/|\nabla \rho|$.}, i.e. in a strongly decreasing density profile the CR pressure would be just as strongly decreasing. For a galactic atmosphere consisting of a dense mid-plane and a rarefied halo, it would imply CR pressure support in the halo is weak. Physically, $P_c$ follows the density profile because the transport speed and collisionless loss rates are both proportional to $v_A$, so the time it takes for CRs to transverse a density scale-height is also the timescale at which it looses energy. Following this logic, if CRs travel faster than it looses energy, then more CRs can escape to the outskirt and CR pressure support there should increase. This can be achieved by increasing diffusion $\kappa$, which causes CR transport to become decoupled with $v_A$. 

In fig.\ref{fig:nobump} we show how the CR pressure profile $P_c$, under various degrees of diffusivity, behaves in an exponentially decreasing density profile. For simplicity we fix the density profile and only evolve the CR pressure and flux through eqn.\ref{eqn:cr_energy} and \ref{eqn:cr_flux}. The CR pressure is fixed on the left boundary and outflow boundary conditions is used on the right side. We initiate density and CR pressure profiles that are exponentially decreasing with the CR diffusion evaluated at each spatial location by $\kappa = \eta\gamma_c L_c v_A$. The CR flux is calculated by eqn.\ref{eqn:cr_flux_steady_state}\footnote{More specifically, the initial profiles we used for generating fig.\ref{fig:nobump} are $P_c = P_{c0} e^{-x}$, $\rho = \rho_0 e^{-2 x/\gamma_c}$ and $F_c = \qty(1 + \eta) \gamma_c P_c v_A/\gamma_c - 1$. The CR scale-height is defined $L_c = P_c/|\nabla P_c|$. The magnetic field is spatially and temporally constant.}. By increasing $\eta$, which is the ratio of the diffusive to streaming flux, the CR pressure increase. The increase in CR pressure also increases the CR heating rate $v_A\cdot\nabla P_c$. The main point from this simple setup is that diffusion causes the $P_c$ profile to become decouple with the density, becoming more dispersed, with $L_c\gg L_\rho$. While we have fixed the CR pressure on the left boundary in this example, in a galactic atmosphere the mid-plane $P_c$ is usually determined by star formation rates (which determines CR production from supernovae) and the model of CR transport used, but the conclusion is always that a more diffusive transport enables CRs to decouple from density and allows a more dispersed $P_c$ distribution. The end result is the halo is more CR pressure supported (see, for example, fig.3 of \citet{farbar18_cr_transport}).

In the streaming dominated regime, the property that $P_c\propto\rho^{\gamma_c/2}$, together with the requirement that CRs can only stream down their gradient, leads to a feature of CR transport known as the ‘bottleneck effect’, predicted analytically by \citet{skilling71_cr_galaxy} and first simulated by \citet{wiener17_cold_clouds}. Imagine having a setup like the one shown in the top of fig.\ref{fig:one_bottle}, where CRs streaming from the left boundary towards the right encounter a density bump in an otherwise hydrostatic-like background. A hydrostatic, smoothly decreasing CR pressure profile like the one shown in blue cannot be in steady state because along the rising side of the density bump, eqn.\ref{eqn:bottleneck_reduce} mandates $P_c$ to be \textit{increasing}. The CRs will slow down at the bump due to decrease in Alfven speed and cause a build up in CR pressure. The build up ceases when the flux of CRs into the well created by the bump equals that going out. What will the final steady state $P_c$ profile be? According to eqn.\ref{eqn:bottleneck_reduce} $P_c$ should be tracing $\rho$, increasing at the rising edge of the bump and falling elsewhere, but this is clearly not the case as shown by simulation (orange curve of the top of fig.\ref{fig:one_bottle}). The reason is, a rising $P_c$ gradient would imply CRs streaming back to the left, contradicting the fact that CR should be fluxing out of the well. The solution is: CRs simply decouple from the gas at the well and free stream out, recoupling at the falling side of the bump. In terms of fluid quantities it means $\nabla P_c = 0$ there, hence the flat plateau as the reader can observe.

In the presence of multiple density bumps the same rationale applies, CRs would bottleneck at each density bumps they encounter, creating a staircase structure like the one shown in the bottom of fig.\ref{fig:one_bottle} (blue curve).\footnote{As explained by \citet{tsung21_staircase}, the ordering of the bump heights along the CRs' path do matter. Specifically, if you place denser bumps after the lighter ones, the CR pressure build up would overwhelm the lighter bump. This stems in crux from CR flux conservation.} Since CR heating is given by $v_A\cdot\nabla P_c$, all the CR heating would be concentrated at the density bumps, where the $P_c$ jumps are. In reality, density bumps of this sort can be formed from in-situ local thermal instability or from CR driven acoustic instabilities \citep{tsung21_staircase,quataert22_cr_wind}, and the staircase would cause CR heating to be concentrated at the bumps, where radiative cooling is likely to be very strong. This way, the surrounding hot gas receives little CR heating and the prospect of supporting an atmosphere from it, as suggested by \citet{guo08_global_stab,wang20_cr_heating_feedback} remains an open question. Following this logic, if there is plenty of cold gas surrounding CR sources, the bottleneck effect would cause most of the CR heating to be screened from the hot gas.

That is the case when streaming transport dominates and the bottleneck is in effect. If diffusion transport dominates, CRs can diffuse out of the bumps easily and there would not be any bottlenecks as CRs are no longer locked with the Alfven waves. Characterizing again the ratio of diffusive to streaming flux by $\eta$, the transition from a well-structured staircase to a smooth, hydrostatic like profile can be clearly seen as $\eta$ transitions across 1 (bottom of fig.\ref{fig:one_bottle}). In the diffusion-smoothed profile CR heating is no longer confined to the bumps, and one could observe, as we shall show in \S\ref{subsec:global_balance}, a great enhancement in the volume averaged CR heating rate.

\begin{figure*}
    \centering
    \includegraphics[width=\textwidth]{cr_heating_2d.png} \\
    \includegraphics[width=\textwidth]{cr_heating_res.png}
    \caption{A similar experiment as that shown in fig.\ref{fig:one_bottle}, but in 2D and with more density bumps scattered around. Again, for illustration purpose, only the CR variables are evolved. Top panel: We show, from top to bottom, the density, CR pressure and CR heating rate. CR diffusivity, characterized by the ratio $\eta$, increases from left to right, where CR heating becomes more distributed. Note that $\eta$ is a function of $x$ (decreasing with $x$), the values of $\eta$ shown is taken at $x=0$. The magnetic field points along the $x$-axis. Bottom panel: The $\eta = 0.01$ case at different resolutions, showing the need to resolve the cold gas to recover the staircase structure and its effect on CR heating.}
    \label{fig:cr_bottle2d}
\end{figure*}

We drive this point more clearly in fig.\ref{fig:cr_bottle2d}, showing the bottleneck effect in 2D. It can be seen, as CR transport becomes more diffusion dominated, the staircase becomes less pronounced and CR heating becomes more distributed rather than being focused at the bumps. High resolution is also needed to manifest the staircase structure and its effect on CR heating.
